How a Small Amount of Data Sharing Benefits Distributed Optimization and Learning : The Upside of Data Heterogeneity

Distributed optimization algorithms are widely used in machine learning. This paper investigates how a small amount of data sharing can improve their performance. Focusing on general linear models, we analyze the effects of data sharing on both primal and primal-dual optimization methods. Our contributions are threefold. First, from a theoretical perspective, we show that minimal data sharing improves algorithmic performance by shifting data from less favorable to more favorable structures. Contrary to the common belief that data heterogeneity is always harmful, we prove that while heterogeneity generally slows convergence in primal methods such as FedAvg and distributed PCG, it can accelerate convergence in primal-dual consensus algorithms like distributed ADMM, Fed-ADMM, and EXTRA by enriching dual dynamics. This reveals a form of duality in how heterogeneity affects different algorithm families. Second, building on this insight, we design a meta-algorithm for minimal data sharing, adaptable to both primal and primal-dual methods. We show that with as little as 1 percent shared data, convergence can be significantly accelerated across machine learning tasks. Finally, we argue from a broader perspective that even limited collaboration can yield large synergies, an idea that transcends the optimization context. Our findings provide both theoretical and practical guidance for improving distributed learning through minimal cooperation and motivate further exploration of cross-agent collaboration in solving complex global learning problems.

==> parking_lot.tex <==
% The reason we introduce the auxiliary variables $\BFt$ is because, when solving for $t_{i,j}$ the problem is much simpler compared with the optimization problem without auxiliary variables. As $t_{i,j}\in(0,1)$, without auxiliary, the problem is not separable across dual variables, and one need to apply for newton method within the blocks in order to perform sub-block optimization. However, with auxiliary variables, optimization for $t_{i,j}$ is separable not only across blocks, but actually across each observations. Hence, one could perform parallel one dimensional search to find the optimal $t_{i,j}$ at each iteration.  


==> temp_PCG.tex <==
We first introduce an approach on constructing local pre-conditioners with shared data, and provide a theoretical improvement on convergence rate for preconditioned conjugate gradient (PCG) with data sharing. We further show that preconditioning is helpful for faster convergence with numerical experiments. Let $\BFX_{\sigma_i}\in \R^{r_i\times p}$ be the selected shared data from agent $i$ with $\BFX_i\in\R^{s\times p}$. We construct local preconditioning matrix with global data share as $\BFH^g_i=(\frac{1}{b}\BFX_i^T\BFX_i+\sum_{j\neq i }\frac{s}{r_i}\BFX^T_{\sigma_i}\BFX_{\sigma_i})^{-1}$. Intuitively, $\BFH_i$ tries to create an estimate of $(\BFX^T\BFX)^{-1}$ with the information from the sampled data. We compare the convergence rate of local preconditioning with shared data to conjugate gradient without preconditioning, and conjugate gradient with local preconditioning of $\BFH_i=(\BFX_i^T\BFX_i)^{-1}$. The following example shows that data sharing is essential for preconditioning. 

==> temp_general_EXTRA.tex <==
Let $(\lambda, \BFxi)$ be the eigenvalue eigenvector pair of $\BFM_E$, with $\BFxi=[\BFu,\BFv]$. Here, note that $(\lambda, \BFxi)$ could be complex. Without loss of generality, we assume unit eigenvector with $\BFxi^*\BFxi=1$. It follows that 
\myeql{\label{extra_eq1}{\begin{bmatrix}
\BFI+\BFP-\rho_E\BFH&\quad -\frac{1}{2}(\BFI+\BFP)+\rho_E\BFH)\\
\BFI &\quad 0
\end{bmatrix}\begin{bmatrix}
\BFu\\
\BFv
\end{bmatrix}=\lambda\begin{bmatrix}
\BFu\\
\BFv
\end{bmatrix}}}
As $\BFu=\lambda\BFv$, with some algebra (\ref{extra_eq1}) implies
\myeql{
(1-\lambda)\rho\BFH \BFv + (\lambda -\frac{1}{2})\BFP \BFv=(\lambda^2+\frac{1}{2}-\lambda)\BFv
}




\newpage

==> temp_previous_proof.tex <==
\subsection{Proof on Theorem \ref{thm_primal_distributed_1} }
\label{app:thm_primal_distributed_1}

To prove Theorem \ref{thm_primal_distributed_1}, notice that the mapping matrix of primal distributed ADMM is given by $\BFM_{p}=\BFI-\BFP-\BFPhi +2\BFPhi \BFP$, where $\BFPhi=\left(\BFI+\frac{1}{\rho_p}\BFD\right)^{-1}$. Let $\lambda\in eig(\BFM_{p})$, and $\BFv$ be the eigenvector associated with $\lambda$, we have $\lambda$ and $\BFv$ satisfies
\myeql{
\label{eq_M}
(\BFI-\BFPhi+(2\BFPhi -\BFI)\BFP)\BFv = \lambda \BFv.
}
For all block $i\in\{1,\dots,b\}$, equation (\ref{eq_M}) becomes
\myeql{
\label{eq_Mi}
(\BFI-\BFPhi_i)\BFv_i + (2\BFPhi_i-\BFI)\bar{\BFv} = \lambda \BFv_i \qquad \forall \ i,}
where $\BFPhi_i=\left(\BFI+\frac{1}{\rho_p}\BFD_i\right)^{-1}$, $\BFv_i\in\R^{p\times1}$ is the $i^{th}$ block of $\BFv$ (the $\{p(i-1)+1,p(i-1)+2,\dots,pi\}^{th}$ row of $\BFv$), and $\bar{\BFv}=\frac{1}{b}\sum^{b}_{i=1}\BFv_i$ is the average of $\BFv_i$.

We first give the proof of a special case where $\BFD_i=\BFD_j$ for all $i,j\in\{1,\dots,b\}$. Later we show that, such data structure is indeed the worst data structure that leads to highest spectrum of mapping matrix $\BFM_{p}$ for the distributed ADMM with fixed $\bar{q}$ and $\underline{q}$ when $\rho_p>\bar{q}$. Let $\tilde{\BFX}$ be the model matrix under the worst case data structure where $\BFD_i=\BFD_j=\frac{1}{b}\tilde{\BFX}^T\tilde{\BFX}$, equation (\ref{eq_Mi}) becomes
\myeql{
\label{eq_Mi_same}
\left(\BFI-\left(\BFI+\frac{1}{b\rho_p}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}\right)\BFv_i + \left(2\left(I+\frac{1}{b\rho_p}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}-I\right)\bar{\BFv} = \lambda \BFv_i \qquad \forall \ i.
}
Let $\BFM_s$ be the primal distributed mapping matrix under $\tilde{\BFX}$, and let $\lambda$ and $\BFv$ be the eigenvalue and eigenvector pairs of $\BFM_s$, the following lemma holds.
\mylemma{
\label{lemma_same}
$$\lambda\neq0 \in \eig(\BFM_s)\quad \Leftrightarrow\quad  \frac{b\rho_p(1-\lambda)}{\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX}) \quad \textup{ or }\quad \frac{b\rho_p\lambda}{1-\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX})$$.
}

\myproof{Suppose $\lambda\neq0 \in \eig(\BFM_s)$, let  $\lambda$ and $\BFv$ be the eigenvalue and eigenvector pairs of $\BFM_s$. Consider the following two cases:

\textbf{Case 1.} $\bar{\BFv}=\frac{1}{b}\sum^{b}_{i=1}\BFv_i\neq0$.

We first show $\lambda\neq0 \in \eig(\BFM_s) \Rightarrow  \frac{b\rho_p(1-\lambda)}{\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX})$. Sum over equation (\ref{eq_Mi_same}) across centers $i$ and take average, 
\myeql{
\label{eq_Mi_same_avg}
\left(\BFI+\frac{1}{b\rho_p}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1} \bar{\BFv}= \lambda \bar{\BFv}.
}
\indent With some algebra 
\myeql{
\label{eq_Mi_same_avg_2}
\tilde{\BFX}^T\tilde{\BFX}\bar{\BFv}= \frac{b\rho_p(1-\lambda)}{\lambda} \bar{\BFv}.
}
\indent Since $\bar{\BFv}\neq0$ and $\lambda\neq0$, we conclude that $\frac{b\rho_p(1-\lambda)}{\lambda} \in eig(\tilde{\BFX}^T\tilde{\BFX})$.

We then show $\lambda\neq0 \in \eig(\BFM_s) \Leftarrow  \frac{b\rho_p(1-\lambda)}{\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX})$. Suppose $\frac{b\rho_p(1-\lambda)}{\lambda} \in eig(\tilde{\BFX}^T\tilde{\BFX})$, let $\frac{b\rho_p(1-\lambda)}{\lambda}$ and $\bar{\BFv}$ be the eigenvalue eigenvector pair of $\tilde{\BFX}^T\tilde{\BFX}$, we have $\lambda\neq0$ and $\bar{\BFv}\neq0$. And it's easy to verify that $\lambda$ and $\BFv=[\bar{\BFv};\dots;\bar{\BFv}]$ satisfies equation (\ref{eq_Mi_same}) for all $i$. Hence, $\lambda\in eig(\BFM_s)$.

\textbf{Case 2. $\bar{\BFv}=\frac{1}{b}\sum^{b}_{i=1}\BFv_i=0$.}

To prove $\lambda\neq0 \in \eig(\BFM_s) \Rightarrow \frac{b\rho_p\lambda}{1-\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX})$, we first claim that if $\lambda$, $\BFv$ are eigenvalue eigenvector pair associated with $\BFM_s$ and $\bar{\BFv}=\frac{1}{b}\sum^{b}_{i=1}\BFv_i=0$, then $\lambda\neq1$, so $\frac{b\rho_p\lambda}{1-\lambda}$ is well-defined. To see this, suppose $\lambda=1\in eig(\BFM_s)$ and the associated eigenvector pair $\BFv$ satisfies $\bar{\BFv}=0$, (\ref{eq_Mi_same}) becomes  
\myeql{
\left(2\left(\BFI+\frac{1}{b\rho_p}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}-\BFI\right)\bar{\BFv} = \left(\BFI+\frac{1}{b\rho_p}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}\BFv_i  \qquad \forall \ i.
}
\indent With some algebra 
\myeql{
\BFv_i=\left(\BFI-\frac{1}{b\rho_p}\tilde{\BFX}^T\tilde{\BFX}\right)\bar{\BFv}  \qquad \forall \ i.
}
\indent As $\bar{\BFv}=0$, $\BFv_i=0$ for all $i$, which contradicts to the fact that $\BFv$ is the eigenvector of $\BFM_s$. Hence when $\bar{\BFv}=0$, if $\lambda\in eig(\BFM_s)$, $\lambda\neq1$. And $\frac{b\rho_p\lambda}{1-\lambda}$ is well-defined.

Take any non-zero $\BFv_i$ (which exists as $\BFv\neq0$), equation (\ref{eq_Mi_same}) becomes 
\myeql{
\left(\BFI-\left(\BFI+\frac{1}{b\rho_p}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}\right)\BFv_i = \lambda \BFv_i.
}
\indent With some algebra
\myeql{
\tilde{\BFX}^T\tilde{\BFX}\BFv_i = \frac{b\rho_p\lambda}{1-\lambda}\BFv_i.
}
\indent Since $\BFv_i\neq0$ and $\lambda\neq1$, we conclude that $ \frac{b\rho_p\lambda}{1-\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX})$.

To prove $\lambda\neq0 \in \eig(\BFM_s) \Leftarrow \frac{b\rho_p\lambda}{1-\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX})$, suppose $\frac{b\rho_p\lambda}{1-\lambda}\in eig(\tilde{\BFX}^T\tilde{\BFX})$, let $\tilde{\BFv}$ be the associated eigenvector pair, $\lambda\neq1$. Let $\BFv$ be such that $\BFv_i=\tilde{\BFv}$ and $\BFv_j=-\frac{1}{b-1}\tilde{\BFv}$ for all $j\neq i$, we have $\bar{\BFv}=\frac{1}{b}\sum^{b}_{i=1}\BFv_i=0$, and it's easy to verify that $\lambda$ and $\BFv$ satisfies equation (\ref{eq_Mi_same}) for all $i$.
}

With Lemma \ref{lemma_same}, let $\tilde{q}\in eig(\tilde{\BFX}^T\tilde{\BFX})$ and $\lambda\in eig(\BFM_s)$, we have $\lambda=\frac{b\rho_p}{b\rho_p+\tilde{q}}$ or $\lambda = \frac{\tilde{q}}{b\rho_p+\tilde{q}}$. As $\tilde{\BFX}^T\tilde{\BFX}$ has fixed largest eigenvalue $\bar{q}$, $\rho_p>\bar{q}$ and $b\geq2$, $\frac{b\rho_p}{b\rho_p+\tilde{q}}>\frac{\tilde{q}}{b\rho_p+\tilde{q}}$. As $\tilde{\BFX}^T\tilde{\BFX}$ has fixed smallest eigenvalue $\underline{q}$, the spectral radius of $\BFM_s$ is given by
\myeql{
\rho(\BFM_s)=\frac{b\rho_p}{b\rho_p+\underline{q}}.
}
\indent To prove Theorem \ref{thm_primal_distributed_1}, we first introduce the following lemma to guarantee that the eigenvalues of mapping matrix $\BFM_{p}$ is in the real space for $\rho_p>\bar{q}$.  
\mylemma{
\label{lemma_real_rho}
Let $\lambda(\BFM_{p})$ be the eigenvalue of mapping matrix $\BFM_{p}$ with $\rho_p>\bar{q}$. $\lambda(\BFM_{p})\in\R$.
}
\myproof{Note $\BFM_{p}=(\BFI-\BFPhi)+(2\BFPhi-\BFI)\BFP$, let $\BFS=2\BFPhi-\BFI$, $\BFS$ is a block diagonal matrix with each diagonal block $i$ given by $\BFS_i=2\left(\BFI+\frac{1}{\rho_p}\BFD_i\right)^{-1}-\BFI$. For $\rho_p>\bar{q}$, $\BFS_i\succ0$ for all blocks $i$. To prove this, let $q_i\in eig(\BFD_i)$, since $\rho_p>\bar{q}$, we have the spectral radius of $\rho\left(\frac{1}{\rho_p}\BFD_i\right)<1$, and the Neumann series exist, with $\BFS_i=2\sum^{n}_{k=0}(-1)^{k}\left(\frac{1}{\rho_p}\BFD_i\right)^{k}-\BFI$, so $\BFS_i$ is a polynomial function of $\BFD_i$, and the eigenvalue of $\BFS_i$ is $\frac{2}{1+q_i/\rho_p}-1>0$.

Since $\BFS_i\succ0$ for all $i$ and $\BFS$ is a block diagonal matrix with $\BFS_i\succ0$, $\BFS\succ0$, and there exists an invertible matrix $\BFB\in\R^{bp\times bp}$ such that $\BFS=\BFB^T\BFB$. Note that $\BFM_{p} \BFS=(\BFI-\BFPhi)\BFS+(2\BFPhi-\BFI)\BFP(2\BFPhi-\BFI)$ and $\BFS\BFM_{p}^T=\BFS(\BFI-\BFPhi)+(2\BFPhi-\BFI)\BFP(2\BFPhi-\BFI)$. Since $\BFS(\BFI-\BFPhi)=-\BFI+3\BFPhi-2\BFPhi^2$, and $\BFPhi$ is symmetric, $\BFS(\BFI-\BFPhi)$ symmetric, and $\BFM_{p}\BFS=\BFS\BFM_{p}^T$. Equivalently, $\BFB^{-1}\BFM_{p}\BFB=(\BFB^{-1}\BFM_{p}\BFB)^T$. Let $\hat{\lambda}$ and $\hat{\BFv}$ be the eigenvalue eigenvector pair of $\BFB^{-1}\BFM_p\BFB$. Since $\BFB^{-1}\BFM_{p}\BFB$ is symmetric, $\hat{\lambda}\in\R$, and  $\BFB^{-1}\BFM_{p}\BFB\hat{\BFv}=\hat{\lambda}\hat{\BFv}$. Hence $\hat{\lambda}$ and $\BFB\hat{v}\neq0$ are the eigenvalue eigenvector pair of $\BFM_{p}$, and $\lambda(\BFM_{p})\in\R$.}

With Lemma \ref{lemma_real_rho}, we could transfer the spectrum of $\BFM_p$ to the eigenvalues of $\BFM_p$, and we prove theorem \ref{thm_primal_distributed_1} by contradiction. From convergence of distributed ADMM (e.g. \cite{eckstein1992douglas}, \cite{he20121}, \cite{ouyang2013stochastic},  \cite{xu2017adaptive}), $\rho(M_p)<1$.

Suppose that $\rho(\BFM_p)> \frac{b\rho_p}{b\rho_p+\underline{q}}$. This implies there exists $\lambda\in eig(\BFM_p)$ and $\lambda\in\left(\frac{b\rho_p}{b\rho_p+\underline{q}}, 1\right)$ or $\lambda\in\left(-1, -\frac{b\rho_p}{b\rho_p+\underline{q}}\right)$. We start to prove by contradiction for the two different cases.

\textbf{Case 1. Suppose $\lambda\in eig(\BFM_p)$ and $\lambda\in\left(\frac{b\rho_p}{b\rho_p+\underline{q}}, 1\right)$.}

\myproof{
Suppose there exists $\lambda \in\left(\frac{b}{b+\lambda_{\min}(\BFX^T\BFX)},1\right)$ and $\lambda$ is the eigenvalue of $\BFM_p$. Let $\BFv=[\BFv_1;\dots;\BFv_i;\dots;\BFv_b]$ be the eigenvector associated with $\lambda$. $\lambda$ and $\BFv$ satisfy equation (\ref{eq_Mi}). Summing over all the $b$ equations and taking the average on both side, we have
\myeql{
\label{eq_Mi1}
-\frac{1}{b}\sum^b_{i=1}\BFPhi_i\BFv_i +\frac{2}{b}\sum^b_{i=1} \BFPhi_i \bar{\BFv} =\lambda \bar{\BFv}.
}
\indent Besides, from equation $(\ref{eq_Mi})$, if $\lambda\in eig(\BFM_p)$, with some algebra
\myeql{
((1-\lambda)\BFI-\BFPhi_i)\BFv_i = (\BFI-2\BFPhi_i)\bar{\BFv}.
}
\indent Following the assumption that $\lambda\in\left(\frac{b\rho_p}{b\rho_p+\underline{q}},1\right)$,  $((1-\lambda)\BFI-\BFPhi_i)^{-1}$ exists. To see this, notice
\myeql{
((1-\lambda)\BFI-\BFPhi_i)^{-1} = -\lambda^{-1}\BFPhi_i^{-1}\left(\BFI-\frac{1-\lambda}{\lambda \rho_p}\BFD_i\right)^{-1}.
}
\indent As $\frac{b\rho_p}{b\rho_p+\underline{q}}>\frac{1}{2}$,  suppose $\lambda\in(\frac{b\rho_p}{b\rho_p+\underline{q}},1)$, $\lambda\in\left(\frac{1}{2},1\right)$, and $\frac{1-\lambda}{\lambda\rho_p}\in(0,1)$. And since $\BFX$ is normalized by its Frobenius norm, $eig(\BFX^T\BFX)\in(0,1)$, so $\eig(\BFD_i)\in(0,1)$, $\left(\BFI-\frac{1-\lambda}{\lambda\rho_p}\BFD_i\right)\succ0$, and the inverse of $\left(\BFI-\frac{1-\lambda}{\lambda\rho_p}\BFD_i\right)$ exists. In fact, following the notation of \cite{plemmons1977m}, $\left(\BFI-\frac{1-\lambda}{\lambda\rho_p}\BFD_i\right)$ is a M-matrix, so its inverse exists with $\left(\BFI-\frac{1-\lambda}{\lambda\rho_p}\BFD_i\right)^{-1}\succ0$ and $\left(\BFI-\frac{1-\lambda}{\lambda\rho_p}\BFD_i\right)$ is inverse positive. Hence $((1-\lambda)\BFI-\Phi_i)^{-1}$ exists, and
\myeql{
\label{eq_vi}
\BFv_i = ((1-\lambda)\BFI-\BFPhi_i)^{-1}(1-2\BFPhi_i)\bar{\BFv}.
}
\indent Notice that $\bar{\BFv}\neq0$. If $\bar{\BFv}=0$, $\BFv_i=0$ for all $i$ and this contradicts with the assumption that $\BFv$ is the eigenvector of $M$. Plugging equation (\ref{eq_vi}) into (\ref{eq_Mi1}), 
\myeql{
\label{eq_vi_in}
\frac{1}{b}\sum^b_{i=1}[2\BFPhi_i -\BFPhi_i((1-\lambda)-\BFPhi_i)^{-1} (I-2\BFPhi_i)]\bar{\BFv}=\lambda\bar{\BFv}.
}
\indent With some algebra,
\myeqmodel{
2\BFPhi_i -\BFPhi_i((1-\lambda)-\BFPhi_i)^{-1} (\BFI-2\BFPhi_i)=-(2\lambda-1)\BFPhi_i((1-\lambda)\BFI-\BFPhi_i)^{-1}\\
=-(2\lambda-1)\BFPhi_i(((1-\lambda)\BFPhi^{-1}_i-\BFI)\BFPhi_i)^{-1}
=(2\lambda-1)\left(\lambda \BFI-\dfrac{(1-\lambda)}{\rho_p}\BFD_i\right)^{-1}.}
\indent Equation (\ref{eq_vi_in}) becomes
\myeql{
\frac{1}{b}\sum^b_{i=1}\left[(2\lambda-1)\left(\lambda \BFI-\frac{(1-\lambda)}{\rho_p}\BFD_i\right)^{-1}\right]\bar{\BFv}=\lambda\bar{\BFv}.
}
\indent Let 
\myeql{f(t|\BFX, \bar{\BFv})=\bar{\BFv}^T\left(\frac{1}{b}\sum^b_{i=1}\left[(2t-1)\left(t \BFI-\frac{(1-t)}{\rho_p}\BFD_i\right)^{-1}\right]\right)\bar{\BFv}-t\bar{\BFv}^T\bar{\BFv},
}
where $\bar{\BFv}^T$ is the transpose of $\bar{\BFv}$ and $\bar{\BFv}\in\R^{p\times1}$. Let $\BFX$ be the associated model matrix of $\BFM_p$, the following relation holds  \myeql{\label{eq_contradiction} \lambda \in eig(\BFM_p)\Rightarrow \textup{there exists } \bar{\BFv}\in\R^{p\times1}\neq0 \textup{ such that } f(\lambda|\BFX, \bar{\BFv})=0.}
\indent To see this, let $\lambda$ and $\BFv$ be the eigenvalue eigenvector pair of $\BFM_p$, since $\lambda\in\R$ and $\BFM_p\in\R^{bp\times bp}$, so $\BFv\in\R^{bp\times1}$. Let $\bar{\BFv}=\sum^{b}_{i=1}\BFv_i$, from equation \ref{eq_vi}, $\bar{\BFv}\in\R^{p\times1}\neq0$, and it's easy to verify that $f(\lambda|\BFX, \bar{\BFv})=0$ for $\lambda\in eig(\BFM_p)$ and $\bar{\BFv}$.

We further prove $\lambda\notin \left(\frac{\rho_p b}{\rho_p b+\underline{q}},1\right)$ by showing that for all $t\in\left(\frac{\rho_p b}{\rho_p b+\underline{q}},1\right)$ and any $\bar{\BFv}\neq0$, $f(t|\BFX, \bar{\BFv})>0$, which contradicts to (\ref{eq_contradiction}), hence if $\lambda\in eig(\BFM_p)$, $\lambda \leq \frac{b\rho_p}{b\rho_p+\underline{q}}$.

Let $\tilde{\BFX}$ be the model matrix such that $\BFD_i=\BFD_j$ for all $\{i,j\}\in\{1,\dots,b\}$ and let $\bar{t}=\frac{b\rho_p}{b\rho_p+\underline{q}}$. By Lemma \ref{lemma_same}, $\bar{t}\in eig(\BFM_s)$, and $f(\bar{t}|\tilde{\BFX},\bar{\BFv})=0$, with $\bar{\BFv}=\frac{1}{b}\sum^{b}_{i=1}\BFv_i$ and $\BFv=[\BFv_1;\dots;\BFv_i;\dots;\BFv_b]$ the associated eigenvector to $\bar{t}$.
We propose the following claims to show that for all $t\in(\bar{t},1)$, $f(t|\BFX, \bar{\BFv})>0$ for all $\BFX$ satisfies assumption \ref{analysis:asmpt_1} and $\bar{\BFv}\neq0$.

\textit{Claim 1: $f(\bar{t}|\tilde{\BFX},\bar{\BFv})\geq 0$ for all $\bar{\BFv}\neq0$.}

\myproof{When $\BFD_i=\BFD_j$ for all $\{i,j\}\in\{1,\dots,b\}$, we have
\myeql{
f(\bar{t}|\tilde{\BFX},\bar{\BFv})=\bar{\BFv}^T\left(\frac{2\bar{t}-1}{\bar{t}}\left(\BFI-\dfrac{1-\bar{t}}{\bar{t}\rho_p}\dfrac{\tilde{\BFX}^T\tilde{\BFX}}{b}\right)^{-1}-\bar{t} \ \BFI\right)\bar{\BFv}.
}
\indent It's sufficient to show that
\myeql{ \label{eq_same_f1}
\frac{2\bar{t}-1}{\bar{t}}\left(\BFI-\dfrac{1-\bar{t}}{\bar{t}\rho_p}\dfrac{\tilde{\BFX}^T\tilde{\BFX}}{b}\right)^{-1}-\bar{t}\ \BFI\succeq 0.
}
\indent Note $\bar{t}=\frac{b\rho_p}{b\rho_p+\underline{q}}$, (\ref{eq_same_f1}) is equivalent as
\myeql{ \label{eq_same_f2}
\left(\BFI-\frac{\underline{q}}{b^2\rho_p^2}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}\succeq \dfrac{b^2\rho^2_p}{b^2\rho^2_p-\underline{q}^2}\BFI.
}
\indent Note that the spectral radius of $\frac{\underline{q}}{b^2\rho_p^2}\tilde{\BFX}^T\tilde{\BFX}$,  $\rho\left(\frac{\underline{q}}{b^2\rho_p^2}\tilde{\BFX}^T\tilde{\BFX}\right)=\frac{\underline{q}\bar{q}}{b^2\rho^2_p}<1$. Hence the Neumann series exists and $\left(\BFI-\frac{\underline{q}}{b^2\rho_p^2}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}$ could be written as the polynomial of $\tilde{\BFX}^T\tilde{\BFX}$. And let $\tilde{q}$ be the eigenvalue of $\tilde{\BFX}^T\tilde{\BFX}$, the eigenvalue of $\left(\BFI-\frac{\underline{q}}{b^2\rho_p^2}\tilde{\BFX}^T\tilde{\BFX}\right)^{-1}$ is given by $\frac{b^2\rho^2_p}{b^2\rho^2_p-\tilde{q}\underline{q}}$, which is lowerbounded by $\frac{b^2\rho^2_p}{b^2\rho^2_p-\underline{q}^2}$. So (\ref{eq_same_f2}) holds and $f(\bar{t}|\tilde{\BFX},\bar{\BFv})\geq 0$.}

\textit{Claim 2: $f(\bar{t}|\BFX,\bar{\BFv})\geq0$, with strict inequality holds when $\BFD_i-\BFD_j$ is non-singular for all $i$ and $j$.}

\myproof{Note for any $\BFX=[\BFX_1,\dots,\BFX_i,\dots,\BFX_b]$ and $\bar{\BFv}\neq0$,
\myeql{
f(\bar{t}|\BFX, \bar{\BFv})=\bar{\BFv}^T\left(\frac{2\bar{t}-1}{\bar{t}} \left[\frac{1}{b}\sum^b_{i=1}\left( \BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\BFD_i\right)^{-1}\right]-\bar{t} \  \BFI\right)\bar{\BFv}.}
\indent We first show that for any $\BFX=[\BFX_1,\dots,\BFX_i,\dots,\BFX_b]$ and $\bar{\BFv}\neq0$,
\myeql{
f(\bar{t}|\BFX,\bar{\BFv})-\bar{\BFv}^T\left(\frac{2\bar{t}-1}{\bar{t}} \left[\frac{1}{b}\sum^b_{i=1}\left( \BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\BFD_i\right)\right]^{-1}-\bar{t} \  \BFI\right)\bar{\BFv}}
\myeql{= \frac{2\bar{t}-1}{\bar{t}}\bar{\BFv}^T \left(\left[\frac{1}{b}\sum^b_{i=1}\left( \BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\BFD_i\right)^{-1}\right]-\left[\frac{1}{b}\sum^b_{i=1}\left( \BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\BFD_i\right)\right]^{-1}\right)\bar{\BFv}\geq0.}
\indent And when $\BFD_i-\BFD_j$ non singular
\myeql{
f(\bar{t}|\BFX,\bar{\BFv})-\bar{\BFv}^T\left(\frac{2\bar{t}-1}{\bar{t}} \left[\frac{1}{b}\sum^b_{i=1}\left( \BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\BFD_i\right)\right]^{-1}-\bar{t} \  \BFI\right)\bar{\BFv}>0.}
\indent Since $\bar{t}>\frac{1}{2}$, $\frac{2\bar{t}-1}{\bar{t}}>0$. It's sufficient to show that
\myeql{
\label{eq_convex1}
\frac{1}{b}\sum^b_{i=1}\left(I-\frac{1-\bar{t}}{\bar{t}\rho_p}\BFD_i\right)^{-1}\succeq \left(\frac{1}{b}\sum^b_{i=1} I-\frac{1-\bar{t}}{\bar{t}\rho_p}\BFD_i\right)^{-1},
}
and when $\BFD_i-\BFD_j$ is non-singular for all $i,j\in\{1,\dots,b\}$, 
\myeql{
\label{eq_convex2}
\frac{1}{b}\sum^b_{i=1}\left(I-\frac{1-\bar{t}}{\bar{t}\rho_p}\BFD_i\right)^{-1}\succ \left(\frac{1}{b}\sum^b_{i=1} I-\frac{1-\bar{t}}{\bar{t}\rho_p}\BFD_i\right)^{-1}.
}
\indent To prove this, we notice that matrix inverse is a (strictly) convex operation. Specifically note that $\left(I-\frac{1-\bar{t}}{\bar{t}\rho_p}\BFD_i\right)^{-1}\succ0$ for all $i$. Following the \cite{brinkhuis2005matrix}, for positive definite matrix $\BFX$ and $\BFY$, with $\alpha\in[0,1]$, the following identity holds
\myeql{
\alpha \BFX^{-1}+(1-\alpha)\BFY^{-1} -[\alpha \BFX+(1-\alpha)\BFY]^{-1}=\alpha(1-\alpha)\BFX^{-1}(\BFY-\BFX)\BFY^{-1}[\alpha \BFY^{-1}+(1-\alpha)\BFX^{-1}]\BFY^{-1}(\BFY-\BFX)\BFX^{-1}.
}
\indent So for $\alpha\in[0,1]$, $\BFX,\BFY\succ0$
\myeql{\label{inv_convex1}
\alpha \BFX^{-1}+(1-\alpha)\BFY^{-1}\succeq [\alpha \BFX+(1-\alpha)\BFY]^{-1},
}
with the following equation holds when $\alpha\in(0,1)$ and $\BFX-\BFY$ non singular
\myeql{\label{inv_convex2}
\alpha \BFX^{-1}+(1-\alpha)\BFY^{-1}\succ [\alpha \BFX+(1-\alpha)\BFY]^{-1}.
}
\indent By induction on applying (\ref{inv_convex1}) and (\ref{inv_convex2}), we prove (\ref{eq_convex1}) and (\ref{eq_convex2}).
We further show that, 
\myeql{
\label{claim_2_ineq}
\bar{\BFv}^T\left(\frac{2\bar{t}-1}{\bar{t}} \left[\frac{1}{b}\sum^b_{i=1}\left( \BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\BFD_i\right)\right]^{-1}-\bar{t} \  \BFI\right)\bar{\BFv}\geq0.}
\indent Note 
\myeql{
\bar{\BFv}^T\left(\frac{2\bar{t}-1}{\bar{t}} \left[\frac{1}{b}\sum^b_{i=1}\left( \BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\BFD_i\right)\right]^{-1}-\bar{t} \  \BFI\right)\bar{\BFv}=\bar{\BFv}^T\left(\frac{2\bar{t}-1}{\bar{t}} \left[\BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\frac{\BFX^T\BFX}{b}\right]^{-1}-\bar{t} \  \BFI\right)\bar{\BFv},}
\indent it's sufficient to show 
\myeql{
\frac{2\bar{t}-1}{\bar{t}} \left[\BFI-\frac{(1-\bar{t})}{\bar{t}\rho_p}\frac{\BFX^T\BFX}{b}\right]^{-1}-\bar{t}\ \BFI\succ0.
}
\indent Following (\ref{eq_same_f2}), this is equivalent as showing 
\myeql{
\label{eq_same_f3}
\left(\BFI-\frac{\underline{q}}{b^2\rho_p^2}\BFX^T\BFX\right)^{-1}\succeq \dfrac{b^2\rho^2_p}{b^2\rho^2_p-\underline{q}^2}\BFI.
}
\indent Similarly, let $q\in eig(\BFX^T\BFX)$, the eigenvalue of $\left(\BFI-\frac{\underline{q}}{b^2\rho_p^2}\BFX^T\BFX\right)^{-1}$ is given by $\frac{b^2\rho^2_p}{b^2\rho^2_p-q\underline{q}}$, which is lowerbounded by $\frac{b^2\rho^2_p}{b^2\rho^2_p-\underline{q}^2}$. So (\ref{eq_same_f3}) holds, hence we prove (\ref{claim_2_ineq}) holds. And we finish the proof on Claim 2.}

%%%% HERE %%%%
\textit{Claim 3: $f(t|\BFX,\bar{\BFv})>0$ for all $t\in(\bar{t},1)$, $\BFX$ and $\bar{\BFv}\neq0$.
}

\myproof{Firstly, notice that given $\BFX$, $f(t|\BFX,\bar{\BFv})$ is a twice differentiable continuous function on $t$ for $t\in(\bar{x},1)$, and $f(1|\BFX,\bar{\BFv})=0$. Furthermore,
\myeql{
\frac{\partial f(t|\BFX,\bar{\BFv})}{\partial t} =\bar{\BFv}^T\left[\frac{1}{b}\sum^b_{i=1}2\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-1}-\frac{1}{b}\sum^b_{i=1} (2t-1)\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-1}\left(\BFI+\frac{1}{\rho_p}\BFD_i\right)\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-1}-\BFI\right]\bar{\BFv}.
}
When $t=1$, 
\myeql{
\frac{\partial f(t|\BFX,\bar{\BFv})}{\partial t}|_{t=1}=-\bar{\BFv}^T\left[\frac{1}{b\rho_p}\BFX^T\BFX\right]\bar{\BFv}<0.
}
And with some algebra, the second order derivative with respect to $t$ is given by
\myeql{
\frac{\partial^2 f(t|\BFX,\bar{\BFv})}{\partial t^2}=\bar{\BFv}^T\left[\frac{2}{b}\sum^b_{i=1}\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-1}\BFM'_i\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-1}\right]\bar{\BFv},
}
where
\myeqmodel{
\BFM'_i &= -2\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)+(2t-1)\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)\left(t\BFI-\dfrac{1-t}{\rho_p}\BFD_i\right)^{-1}\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)\\
& = -2\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)+(2t-1)\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)^2\left(t\BFI-\dfrac{1-t}{\rho_p}\BFD_i\right)^{-1}\\
& = \left(t\BFI-\dfrac{1-t}{\rho_p}\BFD_i\right)^{-1}\left[-2\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)\left(tI-\dfrac{1-t}{\rho_p}\BFD_i\right)^2+(2t-1)\left(t\BFI-\dfrac{1-t}{\rho_p}\BFD_i\right)\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)^2 \right]\left(t\BFI-\dfrac{1-t}{\rho_p}\BFD_i\right)^{-1}.
}
The second and third inequality come from the fact that $\left(\BFI+\frac{\BFD_i}{\rho_p}\right)$ and $\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-1}$ commute.
\myeqmodel{
\left(t\BFI-\dfrac{1-t}{\rho_p}\BFD_i\right)^{-1}\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)&=\dfrac{1}{t}\left(I-\dfrac{1-t}{t\rho_p}\BFD_i\right)^{-1}\left(I+\dfrac{1}{\rho_p}\BFD_i\right)\\
&= \dfrac{1}{t}\sum^{n}_{k=0}\left(\dfrac{1-t}{t\rho_p}\BFD_i\right)^k\left(I+\dfrac{1}{\rho_p}\BFD_i\right)\\
&=\dfrac{1}{t}\sum^{n}_{k=0}\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)\left(\dfrac{1-t}{t\rho_p}\BFD_i\right)^k\\
&=\left(\BFI+\dfrac{\BFD_i}{\rho_p}\right)\left(tI-\dfrac{1-t}{\rho_p}\BFD_i\right)^{-1}.
}
And 
\myeql{
\frac{\partial^2 f(t|\BFX,\bar{\BFv})}{\partial t^2}=\bar{\BFv}^T\left[\frac{2}{b}\sum^b_{i=1}\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-2}\BFM_i\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)^{-2}\right]\bar{\BFv},
}
where
\myeql{
\BFM_i =-2\left(\BFI+\frac{\BFD_i}{\rho_p}\right)\left(tI-\frac{1-t}{\rho_p}\BFD_i\right)^2+(2t-1)\left(t\BFI-\frac{1-t}{\rho_p}\BFD_i\right)\left(\BFI+\frac{\BFD_i}{\rho_p}\right)^2. 
}
Note that $M_i$ is a polynomial function of $\BFD_i$. Let $\BFM_i=P(\BFD_i)$, where
\myeql{
P(x)=\left(\frac{x^2}{\rho^2_p}-1\right)\left(t-\frac{x(1-t)}{\rho_p}\right).
}
Let $\lambda_i\in eig(\BFD_i)$, we have $P(\lambda_i)\in eig(\BFM_i)$. And for $\lambda_i\in(0,1)$ and $t\in\left(\frac{1}{2},1\right)$, $P(\lambda_i)<0$, hence $\BFM_i\prec 0$ for all $i$, and 
\myeql{
\frac{\partial^2 f(t|\BFX,\bar{\BFv})}{\partial t^2}<0, \quad \textup{for } t\in\left(\frac{1}{2},1\right) .
}
Combining the fact that $\bar{t}>\frac{1}{2}$, $f(\bar{t}|\BFX,\bar{\BFv})\geq0$, and $f(1|\BFX,\bar{\BFv})=0$, $\frac{\partial f(t|\BFX,\bar{\BFv})}{\partial t}|_{t=1}<0$, $\frac{\partial^2 f(t|\BFX,\bar{\BFv})}{\partial t^2}<0$ , $f(t|\BFX,\bar{\BFv})>0$ for all $t\in(\bar{t},1)$, and we finish the proof of Claim 3. }

Suppose $\lambda\in eig(\BFM_p)$ and $\lambda\in\left(\frac{b\rho_p}{b\rho_p+\underline{q}}, 1\right)$, there must exist $\bar{\BFv}\neq0$ such that $f(\lambda|\BFX,\bar{\BFv})=0$. However, for all $t\in\left(\frac{b\rho_p}{b\rho_p+\underline{q}}, 1\right)$ and $\bar{\BFv}\neq0$, $f(t|\BFX,\bar{\BFv})>0$. Hence if $\lambda\in eig(\BFM_p)$, $\lambda\notin \left(\frac{b\rho_p}{b\rho_p+\underline{q}}, 1\right)$. And we finish the proof by contradiction for Case $1$.
}

\textbf{Case 2. Suppose $\lambda\in eig(\BFM_p)$ and $\lambda\in\left(-1, -\frac{b\rho_p}{b\rho_p+\underline{q}}\right)$.}

\myproof{Similarly, $((1-\lambda)\BFI-\BFPhi_i)^{-1}$ exists. To see this, notice
\myeql{
((1-\lambda)\BFI-\BFPhi_i)^{-1} = -\lambda^{-1}\BFPhi_i^{-1}\left(\BFI-\frac{1-\lambda}{\lambda \rho_p}\BFD_i\right)^{-1}.
}
\indent As $\left(\BFI-\frac{1-\lambda}{\lambda \rho_p}\BFD_i\right)$ is positive definite, the inverse exists. And 
\myeql{
\label{eq_vi_2}
\BFv_i = ((1-\lambda)\BFI-\BFPhi_i)^{-1}(1-2\BFPhi_i)\bar{\BFv}.
}
\indent Hence we have $\bar{\BFv}\neq0$, as if $\bar{\BFv}=0$, $\BFv_i=0$ for all $i$ which contradicts to $\BFv_i$ is a valid eigenvector. Let 
\myeql{f(t|\BFX, \bar{\BFv})=\bar{\BFv}^T\left( \frac{1}{b}\left[\sum^b_{i=1}\hat{\BFM}_i\right]\right)\bar{\BFv},}
\noindent where
\myeql{
\hat{\BFM}_i=\frac{2t-1}{t}\left( \BFI-\frac{1-t}{t\rho_p}\BFD_i\right)^{-1}-t\ \BFI .
}
\indent The following relation holds 
\myeql{\label{eq_contradiction_2} \lambda \in eig(\BFM_p)\Rightarrow \textup{there exists } \bar{\BFv}\in\R^{p\times1}\neq0 \textup{ such that } f(\lambda|\BFX, \bar{\BFv})=0.}
\indent For $t\in\left(-1, -\frac{b\rho_p}{b\rho_p+\underline{q}}\right)$,  $\BFI-\frac{1-\bar{t}}{\bar{t}\rho_p}\BFD_i\succ0$, so the inverse is also positive definite, and $\frac{2t-1}{t}>0$, so $\hat{\BFM}_i\succ0$ for all $i$, and $f(t|\BFX, \bar{\BFv})>0$ for all $t\in\left(-1,-\frac{b\rho_p}{b\rho_p+\underline{q}}\right)$ and $\bar{\BFv}\neq0$.

Hence if $\lambda\in eig(\BFM_p)$, $\lambda\notin \left(-1, -\frac{b\rho_p}{b\rho_p+\underline{q}}\right)$. And we finish the proof by contradiction for Case $2$.
}

With the previous proof on contradiction, we conclude that$\lambda \notin\left( -\frac{b\rho_p}{b\rho_p+\underline{q}},1\right)$ and  $\lambda \notin \left(-1, -\frac{b\rho_p}{b\rho_p+\underline{q}}\right)$. Hence for $\rho_p>\bar{q}$, the convergence rate of distributed ADMM is upper bounded by $\frac{b\rho_p}{b\rho_p+\bar{q}}$ and the upperbound is achieved when $\BFD_i=\BFD_j$ for all $i,j\in\{1,\dots,b\}$


==> temp_store.tex <==


% simple example
Before introducing the main theorem, we provides an illustrating example on showing how data structure influences the convergence rate under the case matrix conditioning $\underline{q}$ and $\bar{q}$ fixed. Consider a simple case with feature dimensionality $p=1$, number of agents $b=2$ and step size $\rho_p=1$. In the first scenario, the original model matrix $\tilde{\BFX}_i$ and the model matrix after normalizing by Frobenius norm, $\BFX_i$ are given by
\myeql{\label{example_1}
\tilde{\BFX}_1 = 
\begin{bmatrix}0.99\\
0.01
\end{bmatrix}, \quad  \tilde{\BFX}_2=\begin{bmatrix}0.9\\
0.1
\end{bmatrix},\quad {\BFX}_1 = 
\begin{bmatrix}0.7379\\
0.0075
\end{bmatrix}, \quad  {\BFX}_2=\begin{bmatrix}0.6708\\
0.0745
\end{bmatrix}
}
Here, as feature dimensionality $p=1$, $\bar{q}=\underline{q}=1$. If we directly applying Algorithm 1, the linear convergence rate, which is also the spectrum of the linear mapping matrix, is given by $0.6661$. However, consider the second scenario, where we just swap the distribution of data without changing model matrix condition $\underline{q}$ and $\bar{q}$. 
\myeql{\label{example_2}
\tilde{\BFX}_1 = 
\begin{bmatrix}0.99\\
0.9
\end{bmatrix}, \quad  \tilde{\BFX}_2=\begin{bmatrix}0.01\\
0.1
\end{bmatrix},\quad {\BFX}_1 = 
\begin{bmatrix}0.7379\\
0.6708
\end{bmatrix}, \quad  {\BFX}_2=\begin{bmatrix}0.0075\\
0.0745
\end{bmatrix}
}
The convergence rate of applying Algorithm 1 is given by $0.5264$.  In fact, one could show that, for primal distributed ADMM the worst case convergence rate is $0.6667$ and the best convergence rate one could achieve is $0.5$ with $b=2$ and feature dimensionality $p=1$. Here, data structure significantly influences on the convergence rate of primal distributed ADMM from near worst convergence rate to near optimal convergence rate. From this illustrating example, we notice that if different agent shares similar model covariance matrix $\BFD_i=\BFX_i^T\BFX_i$, primal distributed ADMM suffers from convergence.

How Minimal Data Sharing Benefits Distributed Optimization and Learning: The Upside of Data Heterogeneity




While many studies have already studied the impact of global matrix conditioning [\cite{eckstein1992douglas, iutzeler2015explicit, makhdoumi2017convergence}], our work is the first to study how local data structure impacts the convergence speed for distributed ADMM. In order to focus on the impact of local data structure, we first introduce the following assumption on the global data matrix $\BFX$. We assume the global covariance matrix $\BFX^T\BFX$ has fixed conditioning number. Without loss of generality, we further assume that the global covariance matrix is normalized by its Frobenius norm, hence the largest eigenvalue of the global covariance matrix is smaller than $1$ \footnote{In the proof provided in appendix, one would notice that normalizing the global covariance matrix is similar as  adjusting the step size $\rho_p$. Since we allow step size to vary across $(0,\infty)$, normalizing is without loss of generality.}. Fixing the global matrix conditioning allows us to purely focus on the effect on how data structure influences convergence. Also it's worth noticing that any data share across local centers would not influence the conditioning of the global covariance matrix. However, data sharing still significantly changes the local data structure, hence, influencing the convergence speed. 

\myasmp{\label{analysis:asmpt_1} The regressor matrix $\BFX$ is normalized by its Frobenius norm $\|\BFX\|_F$, and the smallest and largest eigenvalue of $\BFX^T\BFX$, $\underline{q}$ and $\bar{q}$ are fixed, with $\BFX^T_i\BFX_i\succ0$ for all $i\in\{1,\dots,b\}$.}

